Ragnar\"ok: A Reusable RAG Framework and Baselines for TREC 2024 Retrieval-Augmented Generation Track

Did you try out the new Bing Search? Or maybe you fiddled around with Google AI~Overviews? These might sound familiar because the modern-day search stack has recently evolved to include retrieval-augmented generation (RAG) systems. They allow searching and incorporating real-time data into large language models (LLMs) to provide a well-informed, attributed, concise summary in contrast to the traditional search paradigm that relies on displaying a ranked list of documents. Therefore, given these recent advancements, it is crucial to have an arena to build, test, visualize, and systematically evaluate RAG-based search systems. With this in mind, we propose the TREC 2024 RAG Track to foster innovation in evaluating RAG systems. In our work, we lay out the steps we've made towards making this track a reality -- we describe the details of our reusable framework, Ragnar\"ok, explain the curation of the new MS MARCO V2.1 collection choice, release the development topics for the track, and standardize the I/O definitions which assist the end user. Next, using Ragnar\"ok, we identify and provide key industrial baselines such as OpenAI's GPT-4o or Cohere's Command R+. Further, we introduce a web-based user interface for an interactive arena allowing benchmarking pairwise RAG systems by crowdsourcing. We open-source our Ragnar\"ok framework and baselines to achieve a unified standard for future RAG systems.

==> tables/raggy2024.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\caption{TREC-RAGgy 2024 query distribution of top-5 categories in topic classification, first-word, and answer type; Long/medium/short denote the answer length.}
    \renewcommand{\arraystretch}{1}
    \small
    {\begin{tabular}{l c@{\hspace{8\tabcolsep}} l c@{\hspace{8\tabcolsep}} l c@{}}
    \toprule
    \multicolumn{2}{l}{\textbf{Topic Classification}} & \multicolumn{2}{l}{\textbf{First Word}} & \multicolumn{2}{l}{\textbf{Answer Type}} \\ \midrule
    Aggregation  & 24.2\% & What  & 37.5\% & Long Answer  & 63.3\% \\ 
    Simple w/ cond. & 23.3\% & How  & 27.5\% & Bullet Points  & 17.5\% \\
    Set  & 20.8\% & Why  & 3.3\% & Multiple Entities  & 14.2\% \\ 
    Simple  & 10.0\% & Is  & 2.5\% & Medium Answer  & 1.7\% \\ 
    Comparison  & 6.7\% & When  & 1.7\% & Short Answer  & 0.8\% \\ \bottomrule
\end{tabular}}\label{tab:query-distribution-trec-raggy}
\end{table}

==> tables/researchy2024.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\caption{TREC-Researchy 2024 query distributions of top-5 categories in query classification and first-word type.}
    \renewcommand{\arraystretch}{1}
    \small
    {\begin{tabular}{l c@{\hspace{8\tabcolsep}} l c@{}}
    \toprule
    \multicolumn{2}{l}{\textbf{Intrinsic Attributes}} & \multicolumn{2}{l}{\textbf{First Word}} \\ \midrule
    Knowledge-Intensive  & 79.8\% & How  & 41.0\%  \\ 
    Multi-faceted & 75.7\% & Why  & 25.5\% \\
    Reasoning-Intensive  & 75.5\% & What  & 15.0\%  \\ 
    Subjective  & 48.5\% & Is  & 5.2\% \\ 
    Assumptive  & 25.7\% & Should  & 2.2\% \\ \bottomrule
\end{tabular}}\label{tab:query-distribution-trec-researchy}
\end{table}
